Value Function Spaces: Skill-Centric State Abstractions for Long-Horizon Reasoning

Reinforcement learning can train policies that effectively perform complex tasks. However for long-horizon tasks, the performance of these methods degrades with horizon, often necessitating reasoning over and chaining lower-level skills. Hierarchical reinforcement learning aims to enable this by providing a bank of low-level skills as action abstractions. Hierarchies can further improve on this by abstracting the space states as well. We posit that a suitable state abstraction should depend on the capabilities of the available lower-level policies. We propose Value Function Spaces: a simple approach that produces such a representation by using the value functions corresponding to each lower-level skill. These value functions capture the affordances of the scene, thus forming a representation that compactly abstracts task relevant information and robustly ignores distractors. Empirical evaluations for maze-solving and robotic manipulation tasks demonstrate that our approach improves long-horizon performance and enables better zero-shot generalization than alternative model-free and model-based methods.

==> analysis.tex <==

\section{Analysis of \algoName for High-Level Planning}
\label{app:proof}

Our analysis is derived from the results presented by \cite{Konidaris2014symbolic}, which show that symbols in an options SMDP are sufficient for high-level planning if they satisfy two conditions: (i) it can represent the \emph{preconditions} for each skill and (ii) it can represent the \emph{image} of each skill-state pair. We first reproduce the definitions of these concepts below, and then show that our skill value function representation satisfies these conditions under some assumptions.

\begin{define}
The \emph{precondition} of a skill $o_i$ is a symbol -- denoting a set of low-level states, -- that represents the states from which $o_i$ will succeed. In the options framework, this refers to its initiation set $\gI_{o_i}$.
\end{define}

\begin{define}
The \emph{image} $\theta(o_i, s)$ of a skill-state pair $\left\{o_i,s\right\}$ is a symbol representing the set of observations that the agent can find itself in after executing skill $o_i$ at state $s$, i.e., $\theta(o_i, s) = \left\{ s' | \exists s \in S, P(s'|s,o_i)>0    \right\}$.
\end{define}



We now show that for a deterministic SMDP $\gM$ with \emph{independent skills} -- where executing skill $o_i$ does not affect the affordances of other skills or their values $V_{o_j} (j \neq i$) -- \algoName can indeed represent these operators, and hence is provably sufficient for high-level planning.

\begin{prop}
Given a deterministic SMDP $\gM$, \algoName can represent the preconditions $\rho(o_i)$ of every skill $o_i \in O$.
\label{prop:precon}
\end{prop}
\begin{proof}
Let $\phi$ denote the event that the agent successfully executed a skill $o_i$, and let $\zeta_{i,t}$ be the reward received by the low-level skill at time step $t$ ($+1$ at success, $0$ otherwise). Then, we have
\begin{equation}
V_{o_i} \left(s \middle| \phi\right) = \E \left[ \sum_{t=1}^{t=\tau} \hat{\gamma}^t \zeta_{i,t} \middle| \phi \right] \geq \hat{\gamma}^\tau \cdot 1
\end{equation}
Therefore, \emph{\algoName can represent preconditions $\rho(o_i)$} by thresholding the skill values
\begin{equation}
\rho(o_i) = \left\{ s \middle| V_{o_i}(s) \geq \hat{\gamma}^\tau \right\}
\end{equation}
\end{proof}


\begin{prop}
Given a deterministic SMDP $\gM$ with independent skills, \algoName can represent the image of a skill $o_i\in O$ from state $s \in S$.
\label{prop:image}
\end{prop}
\begin{proof}
Since the skills are independent, the execution of $o_i$ only affects $Z\left[i\right] = V_{o_i}$. Two cases arise when the agent executes $o_i$ at state $s$:
\begin{enumerate}
    \item \emph{$s \in \rho(o_i)$:} $s$ is in the precondition of $o_i$ and the skill executes successfully, resulting in an updated state $\tilde{Z}\left[i\right]=1$.
    \item \emph{$s \notin \rho(o_i)$:} $s$ is not in the precondition of $o_i$. Since the skills are trained with a sufficiently large $\tau$, this means that the skill is unable to execute successfully and results in an unchanged state $\tilde{Z}\left[i\right]=Z\left[i\right]$.
\end{enumerate}
Therefore, \emph{\algoName can represent the image operator $\theta(\pi, o)$.}
\end{proof}

\begin{result}
Given a deterministic SMDP $\gM$ with \emph{independent} skills, the state abstraction afforded by \algoName is provably sufficient for high-level planning.
\end{result}


The proof follows from the above propositions and \cite[Theorem~1]{Konidaris2014symbolic}. This means that the representation is able to capture all factors of the state that are relevant to interaction with the environment using available low-level skills.

While this result holds for \emph{independent} skills, we often encounter environments where the skills are dependent because they involve interactions with the same object, or otherwise influence each other. 
Interactions like these can be conveniently specified or learned from previous experience in the environment, giving us prior information about the environment. We define a \emph{skill interaction matrix} $\mY(o)$, where $\emY_{ij}(o)$ corresponds to the cumulative reward collected by skill $\pi_j$ while the agent executes skill $\pi_i$ starting from observation $o$.

Given access to this interaction matrix $\mY$ and an SMDP $\gM$, \algoName can represent the effect set for a policy $\pi_i$ by setting updated state $\tilde{Z}[i] = \left\{ \emY_{i1} \ldots, \emY_{ik}, \right\}$, and hence is provably sufficient for high-level planning for an arbitrary set of skills. In practice, we can train a one-step predictive model to learn this interaction matrix (by also using the state information) explicitly, or use a neural network to represent it implicitly from previous experience in the environment.

